Towards visually prompted keyword localisation for zero-resource spoken languages

Imagine being able to show a system a visual depiction of a keyword and finding spoken utterances that contain this keyword from a zero-resource speech corpus. We formalise this task and call it visually prompted keyword localisation (VPKL): given an image of a keyword, detect and predict where in an utterance the keyword occurs. To do VPKL, we propose a speech-vision model with a novel localising attention mechanism which we train with a new keyword sampling scheme. We show that these innovations give improvements in VPKL over an existing speech-vision model. We also compare to a visual bag-of-words (BoW) model where images are automatically tagged with visual labels and paired with unlabelled speech. Although this visual BoW can be queried directly with a written keyword (while our's takes image queries), our new model still outperforms the visual BoW in both detection and localisation, giving a 16% relative improvement in localisation F1.

==> relatedWork.tex <==
\section{Related work}
\label{sec:relatedWork}

Children learn language by using information from co-occurring sensory signals~\cite{dunbar_interspeech_2021}. 
Inspired by this observation, recent
%some
studies~\cite{harwath_jointly_2018, harwath_unsupervised_2016, harwath_learning_2020, harwath_learning_2017, merkx_language_2019} use speech models with visual grounding as pseudo labels. 
These models are trained to retrieve image-caption pairs and therefore aim to learn the overall context of an image and spoken caption.
%Therefore, the objective is not to learn when a word or its corresponding visual object occur in a image-caption pair, 
%which images and captions have the same words or objects in common, 
%but rather which image and caption correspond the most with regards to overall context.
Our aim instead is to obtain a model that can detect if and where a keyword depicted by an image occurs in a spoken caption. 

To do this, \cite{harwath_jointly_2018} uses so-called \textit{matchmaps} %$\mathcal{M}$
to align per frame embeddings to per pixel embeddings.
They quantitatively show that these matchmaps can jointly localise words and objects corresponding to %from
the same concept.
As a result, we use a matchmap model as our starting point for doing
%approach to do
\ac{vpkl} which is derived from the keyword spotting task~\cite{garcia_keyword_2006, szoke_comparison_2005, wilpon_automatic_1990}.
In this spotting task, all utterances from a set that contain a given textual keyword, are returned.
For the new task, we use images instead of textual keywords. 

Previous work~\cite{kamper_visually_2017, kamper_visually_2018} also did this localisation task, but used word embeddings instead of textual keywords. 
To do this, they trained a visually grounded \ac{bow} model by using a visual tagger to extract \ac{bow} keywords for each caption based on its paired image. 
%They do this by training a speech model to detect certain keywords by using a visual tagger to extract keyword targets from a caption's paired image.
Recently, this work was extended to not just detect whether the keyword occurs in the caption, but also to determine where in the caption the word occurs if it was detected~\cite{olaleye_towards_2020, olaleye_attention-based_2021, olaleye_keyword_2022}.
We have the same goal, but we train directly on the image-caption pairs in order to use image keys instead of word embeddings. 
